Co-WIN: Really Winning? Analysing Inequity in India's Vaccination Response

The COVID-19 pandemic has so far accounted for reported 5.5M deaths worldwide, with 8.7% of these coming from India. The pandemic exacerbated the weakness of the Indian healthcare system. As of January 20, 2022, India is the second worst affected country with 38.2M reported cases and 487K deaths. According to epidemiologists, vaccines are an essential tool to prevent the spread of the pandemic. India's vaccination drive began on January 16, 2021 with governmental policies being introduced to prioritize different populations of the society. Through the course of the vaccination drive, multiple new policies were also introduced to ensure that vaccines are readily available and vaccination coverage is increased. However, at the same time, some of the government policies introduced led to unintended inequities in the populations being targeted. In this report, we enumerate and analyze the inequities that existed in India's vaccination policy drive, and also compute the effect of the new policies that were introduced. We analyze these potential inequities not only qualitatively but also quantitatively by leveraging the data that was made available through the government portals. Specifically, (a) we discover inequities that might exist in the policies, (b) we quantify the effect of new policies introduced to increase vaccination coverage, and (c) we also point the data discrepancies that exist across different data sources.

==> text/DISCARDED.tex <==
% \subsection{Data}

% We have used the 2011 census data \cite{census_data} for our analysis. Following are some of the main fields (per district) obtained in the data set - 
% \begin{itemize}
%   \item Number of Households
%   \item Population(Males and Females)
%   \item Literate Males and Females (Literacy Rate)
%   \item Number of Households availing banking services
%   \item Radios/Transistors
%   \item Computers/Laptops with Internet
%   \item Computers/Laptops without Internet
%   \item Landlines
%   \item Mobile Phones
%   \item Bicycles
%   \item Motorcycles/Scooters
%   \item Car/Jeep
% \end{itemize}
% All of the above fields came in three parts - Total , Rural and Urban. The data originally came area wise which we aggregated to district level (35 districts in Maharashtra). The shape files of Maharashtra were converted to geo pandas dataframes with the appropriate district polygons and  appended with the above fields
% \subsection{Analysis - Maharashtra Case Study}
% The next part of data was the centers and their respective
%  The main analysis consisted of observing the change in the number of vaccination centers/ vaccinations made available with for a district and if they had any dependency on factors like spatial position , rural-urban characteristics and the features listed above.

% \subsubsection{Rural vs Urban Areas} 
%  - \newline \textit{\textbf{Number of centers per district}} - The first part of the analysis was comparing the distribution of centers  (more precisely - we took number of centers per 100 households) across maharashtra and comparing that with the rural-urban distribution across the state. The proxy that was used for this is \textbf{the ratio of rural households to the total number of households for the district}. Below \textbf{Figure \ref{fig:rural_urban_num_centers}} shows the comparision

% \begin{figure}[!ht]
% \centering
% \subfloat[ Rural ratio per district. The value at each district is the ratio of rural households to the total households]{{\includegraphics[width=.42\textwidth]{plots_diagrams/micro/Rural_Ratio.jpeg} }}%
% \qquad
% \subfloat[ Number of centers - The value at each district shows the number of centers divided by the total number of households in that district  multiplied by 100]{{\includegraphics[width=.5\textwidth]{plots_diagrams/micro/Num_Centers_per_100.jpeg} }}%
% \caption{Analysis comparing the relation of number of centers per district and the rural ratio per district}
% \label{fig:rural_urban_num_centers}
% \end{figure}

\begin{table}[]
    \centering
    \caption{Pearson's correlation between rural ratio and the vaccines administered/center availability in different states}.
	\label{tab:rural_rat}
	\begin{tabular}{c|cccccc|cccccc}
	%\toprule
	{State} & \multicolumn{6}{c|}{July 22, 2021} & \multicolumn{6}{c}{October 22, 2021}    \\
    {Name} & $C_{v}$ & $C_{c}$ & $N$ 
    & $C^{f}_{v}$ & $C^{f}_{c}$ & $N$ 
    & $C_{v}$ & $C_{c}$ & $N$ & 
    $C^{f}_{v}$ & $C^{f}_{c}$ & $N$ \\
    \midrule
    India & -0.282 &  0.058 & 605 & -0.30 &  0.061 & 364 & -0.291 &  0.157 & 605 & -0.31 &  0.19 & 364\\
    \midrule
    Andhra Pradesh  & -0.76  & -0.329 & 20 & -0.85  & -0.29 & 13 & -0.527  & -0.005 & 20 & -0.67  & 0.063 & 13\\
    Arunanchal Pradesh       &  0.138 &  0.265 & 14 &  0.17 &  0.30 & 9 &  0.132 &  0.132 & 14 &  0.17 &  0.15 & 9\\
    Assam & -0.503 & -0.489 & 25 & -0.68 & -0.50 & 16 & -0.533 & -0.196 & 25 & -0.76 & -0.23 & 16\\
    Bihar & -0.472 & -0.054 & 38 & -0.80 & -0.29 & 23 & -0.69 & -0.122 & 38 & -0.78 & -0.27 & 23\\
    Chhattisgarh & -0.007 &  0.383 & 17 & -0.19 &  0.47 & 11 & -0.007 &  0.33 & 17 & -0.22 &  0.41 & 11\\
    Gujarat &  0.399 &  0.064 & 24 &  0.409 &  0.043 & 15 &  0.494 &  -0.025 & 24 &  0.51 &  -0.046 & 15\\
    Haryana & -0.708 & -0.287 & 20 & -0.695 & -0.232 & 13 & -0.748 & -0.296 & 20 & -0.74 & -0.24 & 13\\
    Himachal Pradesh &  0.052 &  0.538 & 12 &  0.123 &  0.579 & 9 &  0.16 &  0.48 & 12 &  0.233 &  0.529 & 9\\
    Jammu \& Kashmir  &  0.212 &  0.442 & 20 &  0.300 &  0.477 & 13 &  -0.06 &  0.43 & 20 &  -0.048 &  0.478 & 13\\
    Jharkhand & -0.355 &  0.123 & 23 & -0.370 &  0.198 & 15 & -0.662 &  0.105 & 23 & -0.668 &  0.160 & 15\\
    Karnataka &  0.385 &  0.38  & 30 &  0.463 &  0.565  & 19 &  0.531 &  0.33  & 30 &  0.594 &  0.512  & 19\\
    Kerala &  0.489 &  0.394 & 13 &  0.624 &  0.547 & 9 &  0.362 &  0.223 & 13 &  0.563 &  0.396 & 9\\
    Madhya Pradesh & -0.792 & -0.36  & 50 & -0.881 & -0.456  & 31 & -0.802 & -0.29  & 50 & -0.849 & -0.372  & 31\\
    Maharashtra & -0.671 & -0.001 & 33 & -0.663 & 0.048 & 21 & -0.66 & -0.13 & 33 & -0.653 & -0.11 & 21\\
    Odisha & -0.26  & -0.043 & 30 & -0.208  & 0.005 & 19 & -0.12  & -0.043 & 30 & -0.06  & 0.035 & 19\\
     Punjab & -0.401 &  0.118 & 20 & -0.398 &  0.153 & 13 & -0.42 &  0.103 & 20 & -0.411 &  0.162 & 13\\
    Rajasthan &  0.028 & -0.291 & 33 &  0.049 & -0.352 & 21 &  0.089 & -0.27 & 33 &  0.107 & -0.316 & 21\\
    Tamil Nadu & -0.489 & -0.264 & 31 & -0.565 & -0.328 & 19 & -0.419 & -0.32 & 31 & -0.53 & -0.407 & 19\\
    Uttar Pradesh & -0.563 & -0.189 & 66 & -0.562 & -0.193 & 41 & -0.55 & -0.163 & 66 & -0.560 & -0.23 & 41\\
    Uttarakhand &  0.046 &  0.555 & 13 &  0.089 &  0.606 & 9 &  -0.041 &  0.463 & 13 &  -0.39 &  0.545 & 9\\
    West Bengal & -0.819 & -0.68  & 19 & -0.822 & -0.76  & 13 & -0.778 & -0.596  & 19 & -0.80 & -0.65  & 13\\
    \bottomrule
	\end{tabular}
\end{table}

Additionally to see how the vaccination drive is performing over time, we also conduct the same analysis at a later date i.e. 10 months after the drive started and hence significant number of vaccination policies were introduced . We report this result in the same figure as well.

We make the following preliminary observations: The correlation value for the number of centers is close to zero, indicating that the center availability seems to be distributed uniformly across the country. However, at the state-level, we see that some states are more skewed than others. For example, states like Maharashtra, West Bengal, Bihar, Haryana and Uttar Pradesh show significant negative correlation between vaccines administered and the rural ratio, i.e., the number of vaccines administered per 1000 people in districts with a higher rural population is lower. States like Rajasthan, Uttrakhand, Manipur, Mizoram, Himachal Pradesh, and Gujarat have a relatively lower but positive correlation with the number of vaccines, indicating the absence of the negative impact discussed above.

%The input features used for the model are -  the district's area, rural ratio ,log of its population,ratio of males, literacy rate, scheduled caste and scheduled tribe ratio and the ratio of population of different religions. Each feature's \textit{spatial lag} is also used as an input to the model. The spatial lag is the spillover of the value of the feature on the surrounding districts (i.e., change in value for a particular district for unit change in its neighbour's value). Each district's neighbouring districts are found using the Queen-move algorithm\cite{spatial_weights}. This kind of dependence on the spatial arrangement of other data-points is called spatial dependence. To introduce this spatial dependence, each input variable's spatial lag is also included. Therefore, the final equation of the estimating model becomes:

\subsection{CoWIN Portal Data}
\label{sec:prelim_portal}
%We observed the trends of vaccine availability on the CoWIN app as per the CoWIN portal data. There were two key takeaways \MA{what is the prob with takeaways} from the same:
Data obtained from the CoWIN portal API (Sec. \ref{sec:cowin_portal_API}) was the key indicator of vaccine availability capturing how many hourly appointment slots were made available at each vaccination center in each district.
\HL{I vote to remove the following subsection}
\noindent
\textbf{Difference in trends for 18+ and 45+ age group:}
We plot the total number of available appointments returned by the API in every 5 minute window for a one-week period in May for South Delhi district in Fig. \ref{fig:meta45}. There is an evident difference in the behaviour in which slots were booked for the 18+ age group as compared to the 45+ age group. Vaccine slots for the 18+ age group got almost instantaneously booked leading to the sharp spikes we see in the graph. While for 45+ age group, the availability reduces gradually, and in most cases does not reach zero. We observed similar trends in the data pertaining to other districts as well. There are two potential explanations for this behaviour:
\begin{enumerate}
\item Various bots and Twitter accounts have been made available through which individuals can get instantaneous notifications about newly opened slots (Sec. \ref{sec:cowin_api_bot}). Naturally the more tech-savvy younger generation is likely to use these bots to get instant notifications and quickly book their appointments.
\item The 45+ plot rarely shows zero appointment availability meaning that appointments are more readily available for the 45+ age group at any time. This could be because these individuals were not using bots or hesitating to get vaccinated. It could also be that there were generally more slots being made available for older people, or even a discrepancy in the API itself.
\end{enumerate}


\noindent
\textbf{API Reliability for past data:}
\HL{Are we even using this data anywhere.} 

\begin{figure}[]
    \center
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=1\textwidth]{plots_diagrams/vaccines_agewise_South Delhi.png}
    \caption{Vaccine appointment availability for the 18+ and 45+ age groups during a one-week period in May 2021 for South Delhi district.}
    \label{fig:meta45}
  \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
        \centering
    \includegraphics[width=1\textwidth]{plots_diagrams/micro/returned_by_API_time.png}
    \caption{Total daily number of vaccinations based on $d_{hourly}$ between March 8, 2021 and September 14, 2021. }
    \label{fig:time_API}
 \end{minipage}
\end{figure}
